Confidence Matters: Inspecting Backdoors in Deep Neural Networks via Distribution Transfer

Backdoor attacks have been shown to be a serious security threat against deep learning models, and detecting whether a given model has been backdoored becomes a crucial task. Existing defenses are mainly built upon the observation that the backdoor trigger is usually of small size or affects the activation of only a few neurons. However, the above observations are violated in many cases especially for advanced backdoor attacks, hindering the performance and applicability of the existing defenses. In this paper, we propose a backdoor defense DTInspector built upon a new observation. That is, an effective backdoor attack usually requires high prediction confidence on the poisoned training samples, so as to ensure that the trained model exhibits the targeted behavior with a high probability. Based on this observation, DTInspector first learns a patch that could change the predictions of most high-confidence data, and then decides the existence of backdoor by checking the ratio of prediction changes after applying the learned patch on the low-confidence data. Extensive evaluations on five backdoor attacks, four datasets, and three advanced attacking types demonstrate the effectiveness of the proposed defense.

==> 006mitigation.tex <==
% 尽管我们的方法能够检测出许多后门攻击，我们还是需要提出一种能够修复模型的方法。一个可能的选择是，对训练集中所有感染的label的数据，依次用patch进行验证。如果这张图片叠加了patch后被训练好的模型分类为与原始label不一致的标签，那么就将这张图片剔除，否则将这张图片保留。经过这样的筛选后得到一个新的训练数据集，我们在这个新的数据集上重新训练模型。
% 实验结果如图\ref{tab:mitigation}，我们的mitigation方法能够时大部分的攻击影响失效而略有降低重新训练后模型的正确率。但是在Trojan和Multi-Trigger-Multi-Target两个攻击的mitigation不好，前者是因为单个label的数据量太少，产生的patch不能完全过滤掉带有trigger的图片，后者的原因前面已经分析过就是DataCleanse 方法只能找到后门是否存在，无法找到所有infected label。因此在MTMT攻击中只找到了trigger size最小的感染的label，而我们在MTMT感染了0，1，2三个label，也就只能清除某一个label带来的影响。

When checking that the model has a backdoor, it needs to remove trigger samples from the training data, and retrain the model. The data cleaning part will be discussed in \textbf{evaluation part}.

Then, mitigation module will be applied to the target label to remove the samples with trigger. Finally, the model will be trained on cleaned data set


Although Data Cleanse can detect many backdoor attacks, we still need to propose a method that can repair the model. One possible choice is to verify the data of all infected labels in the training set with patches in turn. If the image superimposed with the patch is classified to a label which is inconsistent with the original label, then the image will be removed, otherwise the image is retained. After such cleaning, a new training data set is obtained, and we retrain the model on this new data set. The experimental results are shown in figure \ref{tab:mitigation}. Our mitigation method can invalidate most of the attack effects and slightly reduce the accuracy of the model after retraining. However, the mitigation of the Trojan and Multi-Trigger-Multi-Target attacks is not good. The former is because the number of the a single label data is too little so that the generated patch are not completely cover the trigger area and hard to filter out some of the images with the trigger. The reason for the latter has been analyzed before that the Data Cleanse method can only find whether the backdoor exists, and can only find one infected labels whose trigger is smallest. Therefore, the attack success rate of the retrained model attacked by MTMT is reduced to 67.06\%.  
\input{tables/table_mitigation}







